Towards remote fault detection by analyzing communication priorities

The ability to detect faults is an important safety feature for event-based multi-agent systems. In most existing algorithms, each agent tries to detect faults by checking its own behavior. But what if one agent becomes unable to recognize misbehavior, for example due to failure in its onboard fault detection? To improve resilience and avoid propagation of individual errors to the multi-agent system, agents should check each other remotely for malfunction or misbehavior. In this paper, we build upon a recently proposed predictive triggering architecture that involves communication priorities shared throughout the network to manage limited bandwidth. We propose a fault detection method that uses these priorities to detect errors in other agents. The resulting algorithms is not only able to detect faults, but can also run on a low-power microcontroller in real-time, as we demonstrate in hardware experiments.

==> PredictiveTriggering/PredictiveTriggering.tex <==
\section{Event triggered control over multi-hop networks}
\subsection{Stability analysis}
For our stability analysis, we assume that agents $j$ and $m$ have the same estimate of agent $i$'s state $\stateest{i j}{k} = \stateest{i m}{k},~\forall m,j,i\in\left\{1, \cdots, N\right\}$. This property is critical as interagent error has shown to lead to instability in similar scenarios \cite{Trimpe_2014}. The communication protocol mixer has shown to be very robust in past experiments includes a technique that is able to detect if every agent received the messages. This allows to only use received messages, when all agents received them and thus eliminating the occurrence of interagent error. \ag{Thats not implemented, but will be implemented in the future (maybe), perhaps we should just say we neglect message loss, because our protocol is very reliable.}\\
To simplify the notation we will only use one index for estimation error, estimated state $\stateest{i}{k}= \stateest{i j}{k} = \stateest{i m}{k}$ and scheduling $\rec{i}{k}$ in the following.

When appropriate controller gains $\matF{ij}$ are chosen the multi-agent system is stable.
As a stability measure we select mean square boundedness (MSB) \cite{Baumann_2020, Ramponi2010}.
\begin{definition}
	\label{def:msb}
	The system (\ref{eq:systemdefinition}) is called MSB, when there exist $\bar{\epsilon}>0$ and $\rho\of{\epsilon}$ such that for every $\epsilon>\bar{\epsilon}$ $\twonorm{\state{i}{0}}^2<\rho$ implies $\sup_{k\geq0}\EX\of{\twonorm{\state{i}{k}}^2\given\state{i}{0}}\leq\epsilon$
\end{definition}
To proof MSB the following lemmas are useful:
\begin{lemma}
	\label{lem:boundnessmarkovchain}
	Consider a Markov chain $\vephi$ with state $\vex\in\mathbb{X}\subseteq\mathbb{R}^n$. If there exists a $\tilde{K}>0$ such that $\EX\ofs{\twonorm{\vex\tp{\tilde{K}}}^2\given\vex\tp{0}}\leq C, \forall \vex\tp{0}\in\mathbb{X}$, then for all $K\geq\tilde{K}$ $\EX\ofs{\twonorm{\vex\tp{K}}^2\given\vex\tp{0}}\leq C, \forall \vex\tp{0}\in\mathbb{X}$.
\end{lemma}
\begin{proof}
It is 
\small
\begin{equation}
	\begin{split}
&\EX\ofs{\twonorm{\vex\tp{K}}^2\given\vex\tp{0}}	= \int\limits_{\mathbb{X}}\twonorm{\vex\tp{K}}^2 p\of{\vex\tp{K}\given \vex\tp{0}}\diff\vex\tp{K}\\
&\medmath{=\int\limits_{\mathbb{X}}\twonorm{\vex\tp{K}}^2\int\limits_{\mathbb{X}}p\of{\vex\tp{K}\given \vex\tp{K-\tilde{K}}}p\of{\vex\tp{K-\tilde{K}}\given \vex\tp{0}}\diff\vex\tp{K-\tilde{K}}\diff\vex\tp{K}}\\
&\medmath{=\int\limits_{\mathbb{X}}\int\limits_{\mathbb{X}}\twonorm{\vex\tp{K}}^2 p\of{\vex\tp{K}\given \vex\tp{K-\tilde{K}}}\diff\vex\tp{K}p\of{\vex\tp{K-\tilde{K}}\given \vex\tp{0}}\diff\vex\tp{K-\tilde{K}}}\\
&\leq\int\limits_{\mathbb{X}}C p\of{\vex\tp{K-\tilde{K}}\given \vex\tp{0}}\diff\vex\tp{K-\tilde{K}}\\
&=C.
\end{split}
\end{equation}
\normalsize
\ag{for the second line: has the markov chain to have markov property?}
\end{proof}
\begin{lemma}
	Consider a Markov chain $\vephi$ with state $\vex\in\mathbb{X}\subseteq\mathbb{X}$. If there exists a $\tilde{K}>0$ such that $\EX\ofs{\twonorm{\vex\of{\tilde{K}}}^2\given\vex\of{0}}\leq C, \forall \vex\of{0}\in\mathbb{X}$ and $\EX\ofs{\twonorm{\vex\of{k}}^2\given\vex\of{0}}\leq \infty, \forall \vex\of{0}\in\mathbb{X}, \forall k > 0$, then the Markov chain is MSB.
\end{lemma}
\begin{proof}
	\label{lem:MSBlemma}
	Because of lemma \ref{lem:boundnessmarkovchain} we know that for all $K\geq\tilde{K}$ $\EX\ofs{\twonorm{\vex\tp{K}}^2\given\vex\tp{0}}\leq C, \forall \vex\tp{0}\in\mathbb{X}$. Thus we know $\forall \vex\tp{0}\in\mathbb{X}$
	\small
	\begin{equation}
		\begin{split}
		\EX\ofs{\twonorm{\vex\tp{k}}^2\given\vex\tp{0}} &\leq \medmath{\max\left\{C, \max_{\tilde{k}\in\left\{0,\cdots,K-1\right\}}	\EX\ofs{\twonorm{\vex\tp{\tilde{k}}}^2\given\vex\tp{0}}\right\}}\\
		& = \tilde{C}
		\end{split}
	\end{equation}
	\normalsize
	Select now $\tilde{\epsilon}=\tilde{C}$. Then for any $\epsilon>\tilde{\epsilon}$ and an arbitrary function $\rho\of{\epsilon}$ for any $\twonorm{\vex\tp{0}}^2<\rho\of{\epsilon}$
	\begin{equation}
	\EX\ofs{\twonorm{\vex\tp{k}}^2\given\vex\tp{0}} \leq \tilde{C} < \epsilon	
	\end{equation}
\end{proof}
In the following we will use this lemma to show that the estimation errors of the observers are MSB. We just have to show that the second order norm of the estimation error is at some time bounded by a constant.\\
Due to the triggering the estimation error is not normal distributed. Its dynamics are
%\begin{equation}
%	\label{eq:estError}
%	\begin{split}
%		&\errorest{i}{k+1} = \stateest{i}{k+1} - \state{i}{k+1} \\&= \begin{cases}
%			\matAti{l}\errorest{i}{k} + \vev\uli{i}\tp{k} & \text{if~}\rec{i}{k} = 0\\
%			\ve{v}\uli{i}\tp{k} & \text{if~}\rec{i}{k} = 1
%		\end{cases}
%	\end{split}
%\end{equation}
Key point of our stability analysis is that once an agent $i$ sends its state, its estimation error $\errorest{i}{k}$ gets bounded by a constant only dependent of the time after the scheduled slot. 
\begin{lemma}
	\label{lem:lemmaboundness}
	Let the error $\errorest{i}{k}$ be bounded by $\EX{\twonorm{\errorest{i}{k}}^2}<\alpha$ and assume the system is not scheduled a slot in the interval $\left[k, k+\kappa-1\right]$, then there exist $\beta\uli{i}\of{\kappa, \alpha}$ such that \begin{equation}
		\EX\ofs{\twonorm{\errorest{i}{k+\kappa}}^2\given \errorest{i}{k}, \rec{i}{k} = 0, \cdots, \rec{i}{k+\kappa-1} = 0 }<\beta\uli{i}\of{\kappa, \alpha}
	\end{equation}.
\end{lemma}
\begin{proof}
	Main idea of the proof is that the information \ldq agent $i$ not scheduled a slot\rdq{} gives information about its estimation error (negative information \cite{Sijs2013}).
	When the system was not allowed to send, we know that 
	\db{hat es einen bestimmten Grund, dass du die time steps hochstellst (also $x^{(k)}$ anstelle von $x(k)$)? Ich denke zusammen mit dem transpose Operator koennte das verwirrend sein}
	\ag{Dadurch werden die Formeln etwas kürzer (auf die physikalische Länge im Text bezogen). Wenn das zu verwirrend ist, stelle ich es um.}
	\begin{equation}
		\begin{split}
			&\errorest{i}{k+\tau}{}^\transp\matQ{i}\errorest{ij}{k+\tau} + \epsilon\ul{i} \\&\leq \max_{\ell\in\left\{1,\cdots,N\right\}~\ell\neq i} \errorest{\ell}{k+\tau}{}^\transp\matQ{\ell}\errorest{\ell}{k+\tau} + \epsilon\ul{\ell} = g\tp{k+\tau},
		\end{split}
	\end{equation}
	for all $\tau\in\left\{0,\dots,\kappa-2\right\}$. We define $\ve{g} = \left[ g\tp{k}, \cdots, g\tp{k+\kappa-2}\right]$. This vector is stochastic and its distribution based on the other agents. We will no show that for every single possible value $	\EX\ofs{\twonorm{\errorest{i}{k+\kappa}}^2\given \errorest{i}{k}, \rec{i}{k} = 0, \cdots, \rec{i}{k+\kappa-1} = 0, \ve{g}}$ is bounded.\\
	For every $\tau$ we arbitrary set $g\tp{k+\tau}=\max\left\{\min_{\ell\in\left\{1,\cdots,N\right\}~\ell\neq i}\epsilon\ul{\ell},~ \epsilon\ul{ij} \right\} = g\ul{0}$ or letting $g\tp{k+\tau}\rightarrow\infty$ respectively e.g. $\ve{g}=\left[g\ul{0}, g\ul{0},\rightarrow \infty, g\ul{0},\rightarrow \infty \cdots\right]$. The boundedness of the expectation of every other $\ve{g}$ follows directly out of the continuity of $\EX\ofs{||\errorest{ij}{k+\kappa}||_2^2\given\errorest{ij}{k}, \rec{ij}{k\cdots k+\kappa-1}=0, \ve{g}}$ regarding $\ve{g}$.\\
	We observe, that at some time $k+a$, the corresponding entry in $\ve{g}$ is equal to $g\ul{0}$ and after this entry every other entry goes to infinity or the vector ends. (except for the case where every entry goes to infinity, which will be investigated afterwards). Thus we can write
	\begin{equation}
		\twonorm{\errorest{i}{k+a}}^2 \leq \frac{g\ul{0} - \epsilon\uli{i}}{\lambdaminof{\matQ{i}}},
	\end{equation}
	where $\lambdaminof{\matQ{i}}>0$ is the smallest eigenvalue of $\matQ{i}$, which directly follows if we insert $g\ul{0}$ into (\ref{eq:priority}) and solve for $\twonorm{\errorest{i}{k+a}}^2$.  It follows
	\small
	\begin{equation}
		\label{eq:argumentationaunequalzero}
		\begin{split}
			&\EX\ofs{||\errorest{i}{k+\kappa}||_2^2\given\errorest{i}{k}, \rec{i}{k\cdots k+\kappa-1}=0, \ve{g}} \\
			&=\medmath{\EX\left[\twonorm{\matAti{i}^{\kappa-a}\errorest{i}{k+a} + \sum_{\tau=0}^{\kappa-1-a}\matAti{i}^{\tau}\processnoise{l}{k+\kappa-1-a-\tau}}^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}\right]}\\
			&=\EX\ofs{\twonorm{\matAti{i}^{\kappa-a}\errorest{i}{k+a}}^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}} \\
			&+\EX\ofs{\twonorm{\sum_{\tau=0}^{\kappa-1-a}\matAti{i}^{t}\processnoise{i}{k+\tau-1-a-\tau}}^2\given\rec{i}{k\cdots k+\tau-1}=0, \ve{g}}\\
			&\leq\frac{g\ul{0} - \epsilon\uli{i}}{\lambdaminof{\matQ{i}}} + \tr\of{\sum_{\tau=0}^{\kappa-1-a}\matAti{i}^t\matV{i}\left(\matAti{i}^t\right)^\transp} = \beta\uli{i}\of{\kappa},
		\end{split}
	\end{equation}
	\normalsize
	because the last entries of $\ve{g}$ go to infinity and thus the corresponding noise is normal distributed with mean zero and independent of $\errorest{i}{k+a}$.\\
	For the case, where the whole vector $\ve{g}$ goes to infinity we get
	\small
	\begin{equation}
		\begin{split}
			&\EX\ofs{||\errorest{i}{k+\kappa}||_2^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}} \\&\medmath{=\EX\ofs{\twonorm{\matAti{i}^{\kappa}\errorest{i}{k} +\sum_{\tau=0}^{\kappa-1}\matAti{i}^{\tau}\processnoise{i}{k+\kappa-1-\tau}}^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}}}\\
			&=\EX\ofs{\twonorm{\matAti{i}^{\kappa}\errorest{i}{k}}^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}} \\
			&+\EX\ofs{\twonorm{\sum_{\tau=0}^{\kappa-1-a}\matAti{i}^{\tau}\processnoise{i}{k+\kappa-1-\tau}}^2\given\rec{i}{k\cdots k+\kappa-1}=0, \ve{g}}\\
			&\leq\twonorm{\matAti{i}^{\kappa}}^2\alpha+\tr\of{\sum_{\tau=0}^{\kappa-1}\matAti{i}^\tau\matV{i}\left(\matAti{i}^\tau\right)^\transp},\\
		\end{split}
	\end{equation}
	\normalsize
	where $\alpha$ is constant.
	\db{With $\alpha$ and $\beta$ you are here using two new variables that have not been defined prior as far as I have seen. So both should at least shortly be introduced}\ag{they are first defined in the lemma. Do I have to explicitly explain them?}
	\db{Yes, this is something reviewers like to complain about. Something like ``where $\alpha$ is a constant'' is sufficient.}
	We have showed show that for every combination of  entries of $\ve{g}$ being either constant or going to infinity $\EX\ofs{||\errorest{i}{k+\kappa}||_2^2\given\errorest{i}{k}, \rec{i}{k\cdots k+\kappa-1}=0, \ve{g}}$ is bounded. Therefor the boundedness of $\EX\ofs{||\errorest{i}{k+\kappa}||_2^2\given\errorest{i}{k}, \rec{i}{k\cdots k+\kappa-1}=0}$ follows directly out of the continuity of the expected value regarding $\ve{g}$.\\
\end{proof}

Whenever we can upper bound the expectation of the quadratic estimation error by a constant, this lemma states that its estimation error is also bounded in the future. The value of this bound is only dependent on the time and not the other agent's state or estimation errors. This lemma helps us unravel the dependencies between other agents estimation errors.\\
With this we can prove mean square stability of the estimation error. 

\begin{lemma}
	The estimation error (\ref{eq:estError}) of system (\ref{eq:systemdefinition}) is MSB.
\end{lemma}
\begin{proof}
	We build a Markov chain by putting every error $\errorest{i}{k}$ into one state. Because their future also depends on the errors one timestep back (they are responsible for the triggering of the messages received at $k+1$), we also augment the state by time delays $\errorest{i}{k-1}$ such that the Markov chain fulfills the Markov property. In order to proof stability for the whole system, we just show that the expectation of the second order norm at time $L>2N/M$ is bounded and use lemma \ref{lem:MSBlemma} to show MSB.\\
	We show that for every realization  of the scheduling $\setS = \left\{\rec{i}{k+\kappa}:~i\in\left\{1, \cdots, N\right\}, \kappa\in\left\{0, L\right\} \right\}$ $	\EX\ofs{\ve{e}\tp{L}\given \setS, \ve{e}\tp{0} }$ is upper bounded by a constant. The upper boundedness of $\EX\ofs{\ve{e}\tp{L}\given \ve{e}\tp{0} }$ follows directly.\\
	Our proof uses the same technique as in \cite{Mamduhi2015} \cite{Mamduhi_2017}\cite{PredictiveTriggering}
	We split the agent into two different sets
	\begin{enumerate}
		\item $\cone$ every agent that was assigned a slot at least once in the interval $\left[k, k+L-1\right]$. Or more formal $\cone = \left\{i\in\left\{1, ..., N\right\}: \exists t\in \left\{\left\{k, ..., k+L-1\right\} s.t. \gamma\uli{i}\of{t} = 1\right\}\right\}$. Note that this set is never empty.
		\item $\ctwo = \left\{1, ..., N\right\}\setminus \cone$ every agent that was not able to send during the same time period. 
	\end{enumerate}
	When an agent $i\in \cone$ had the opportunity to last send at time $k+\ri{i}-1$, we know
	\begin{equation}\veerr\uli{i}\of{k+\ri{i}}=\processnoise{i}{k+\ri{i}-1}
	\end{equation}
	We can construct an artificial error $\errart{i}{k+\ri{i}-1}=\ve{0}$, with $\errart{i}{k+\ri{i}}=\veerr\uli{i}\of{k+\ri{i}}, \cdots$ and due to lemma \ref{lem:lemmaboundness} we know 
	\begin{equation}
		\label{eq:csupperbound}
		\EX\ofs{||\errorest{i}{k+L}||_2^2\given\veerr\tp{k}, \cone} \leq \tilde{\beta}\uli{i}\of{L}
	\end{equation}
	For every agent in $\cone$ we showed that its expected squared estimation error is bounded by a constant. This result is also important to show the boundedness of the expected squared estimation error of agents in the second set.\\
	Because we have chosen $L>2N/M$ every agent should have had the opportunity to send at least two times \footnote{Due to the delay of our scheduling algorithm agents usually send two times in a row.}. If there are agents in $\ctwo$, there are agents in $\cone$ that where allowed to send three times. So at some time $k+\di{i}$ one agent $i\in\ctwo$ is scheduled for the at least third (and last) time. Thus at this time the priority of every agent $j$ in $\ctwo$ is lower than the priority of agent $i$
	\begin{equation}
		\begin{split}		&\errorest{j}{k+\di{i}}{}^\transp\matQ{j}\errorest{j}{k+\di{i}} \leq \errorest{i}{k+\di{i}}{}^\transp\matQ{i}\errorest{i}{k+\di{i}} + \deltai{ij},
		\end{split}
	\end{equation}
	where $\deltai{ij} = \epsilon\uli{i}-\epsilon\uli{j}$ 
	and thus
	\begin{equation}
		\label{eq:twonormerrorbound}
		\begin{split}
			&\EX\ofs{\twonorm{\errorest{j}{k+\di{i}}}^2\given \veerr\tp{k}, \cone}\\ &\leq \frac{\twonorm{\matQ{i}}}{\lambdaminof{\matQ{j}}}\EX\ofs{\twonorm{\errorest{i}{k+\di{i}}}^2\given\veerr\tp{k}, \cone} + \frac{\deltai{ij}}{\lambdaminof{\matQ{j}}},
		\end{split}
	\end{equation}
	We can use the same argumentation as for equation (\ref{eq:csupperbound}) to show that $\EX\ofs{\twonorm{\errorest{i}{k+\di{i}}}^2\given\veerr\tp{k}, \cone}$ is bounded by a constant and thus also $\EX\ofs{\twonorm{\errorest{j}{k+\di{i}}}^2\given \veerr\tp{k}, \cone}$ is bounded by a constant. Using lemma \ref{lem:lemmaboundness}, we get
	\begin{equation}
		\EX\ofs{||\errorest{j}{k+L}||_2^2\given\tveerr\of{k}, \cone} \leq \tilde{\alpha}\uli{j}\of{L}
	\end{equation}
	The same argumentation can be done for the time delayed estimation errors $\errorest{j}{k-1}$.
	We now have showed that the expectation of the second moment of every estimation error is bounded. Because of lemma \ref{lem:MSBlemma}, the estimation error is MSB.
\end{proof}

We now proof stability of the multiagent system. Combining the states $\state{i}{k}$ to one state and merging the state, input and control matrices together, we get the overall system dynamics $\left(\matA{}, \matB{}\right)$ with linear controller $\matF{}$.
\begin{theorem}
	If the matrix $\matA{} + \matB{}\matF{}$ has only eigenvalues within the unit circle, the presented heterogeneous multiagent system can be stabilized using the predictive triggered control architecture.
\end{theorem}

\begin{proof}
	The agents dynamics can be rewritten as
	\begin{equation}
		\begin{split}
			\state{i}{k+1} &= \left(\matA{i} + \matB{i}\matF{ii}\right)\state{i}{k} + \sum_{l = 1, l \neq i}^{N}\matB{i}\matF{il}\stateest{l}{k} + \vev\uli{i}\tp{k}\\
			&= \left(\matA{i} + \matB{i}\matF{ii}\right)\state{i}{k} + \sum_{l = 1, l \neq i}^{N}\matB{i}\matF{il}\state{l}{k} \\
			&- \sum_{l = 1, l \neq i}^{N}\matB{i}\matF{il}\errorest{l}{k} + \vev\uli{i}\tp{k}.
		\end{split}
	\end{equation}
	The overall system dynamics are
	\begin{equation}
		\begin{split}
			\state{}{k+1} &= \left(\matA{} + \matB{}\matF{}\right)\state{}{k} - \widetilde{\matB{}\matF{}}\erroragents{}{k} + \vev\uli{}\tp{k}
		\end{split}
	\end{equation}
	We know the estimation error and the process noise is MSB. MSB of the controlled system follows directly from the BIBO property of the global system $\left(\matA{} + \matB{}\matF{}, \widetilde{\matB{}\matF{}}\right)$ \cite[Ch. 7.6d]{Frank2012}\cite{PredictiveTriggering}.\\
\end{proof}
